Online Political Discourse in the Trump Era

We identify general trends in the (in)civility and complexity of political discussions occurring on Reddit between January 2007 and May 2017 -- a period spanning both terms of Barack Obama's presidency and the first 100 days of Donald Trump's presidency. We then investigate four factors that are frequently hypothesized as having contributed to the declining quality of American political discourse -- (1) the rising popularity of Donald Trump, (2) increasing polarization and negative partisanship, (3) the democratization of news media and the rise of fake news, and (4) merging of fringe groups into mainstream political discussions.

==> Makefile <==
# Makefile for LaTeX files

# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile

# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.

# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 

# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips
DVIPDF  = dvipdft
L2H	= latex2html
GH	= gv

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

DATE=$(shell date +%Y-%m-%d)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

# These are OK

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)

# These are not

#BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))


define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

define run-pdflatex
	LATEX=pdflatex
	@$(run-latex)
endef

define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef

define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef

define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef

define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef

all 	: $(TRG)

.PHONY	: all show clean ps pdf showps veryclean

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)

veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~

# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 

include $(SRC:.tex=.d)

# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)

$(PSF)	: %.ps : %.dvi
	  @$(DVIPS) $< -o $@

#$(PDF)  : %.pdf : %.dvi
#	  @$(DVIPDF) -o $@ $<
# To use pdflatex, comment the two lines above and uncomment the lines below
$(PDF) : %.pdf : %.tex
	@$(run-pdflatex)


show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done

showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done

ps	: $(PSF) 

pdf	: $(PDF) 

# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)



######################################################################
# Define rules for EPS source files.

# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12

#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
#%.eps: %.png
#	$(OUTDATED)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))

